A Simple LP-Based Approximation Algorithm for the Matching Augmentation Problem

The Matching Augmentation Problem (MAP) has recently received significant attention as an important step towards better approximation algorithms for finding cheap $2$-edge connected subgraphs. This has culminated in a $\frac{5}{3}$-approximation algorithm. However, the algorithm and its analysis are fairly involved and do not compare against the problem's well-known LP relaxation called the cut LP. In this paper, we propose a simple algorithm that, guided by an optimal solution to the cut LP, first selects a DFS tree and then finds a solution to MAP by computing an optimum augmentation of this tree. Using properties of extreme point solutions, we show that our algorithm always returns (in polynomial time) a better than $2$-approximation when compared to the cut LP. We thereby also obtain an improved upper bound on the integrality gap of this natural relaxation.

==> preliminaries.tex <==
\hl{appendix or here??}
Given a graph $G=(V, E)$ and a rooted tree $T\subseteq E$, we say an arc $e \in E \setminus T$ is an \textit{up-link} or \textit{back-edge} if $e=uv$, where $u$ is an ancestor of $v$ in $T$. Other links are called \textit{cross-edges}.

In an instance of FAP, with input graph $G=(V,E)$ and forest $F$, a common approach, which we exploit the algorithm, is to connect the matching into a tree $T$ and then augment $T$ into a 2-Edge Connected Sub-graph. The linear programming relaxation of the associated tree augmentation problem is given by $LP(G, T)$.

Since we select $T$ to be a DFS we know that the set of up-links of $G$ with respect to $T$ is precisely $E \setminus T$. In such instances the feasible region of $LP(G,T)$ is integral, as stated in Lemma \ref{lem:integral_DFS_augmentation}.
This holds as the problem formulated can be formulated minimum-cost circulation. We note that the result is used in \cite{momke2016removing} and \cite{cohen20131+}.
\begin{lemma}\label{lem:integral_DFS_augmentation}
Suppose we are given a graph $G=(V,E)$ a spanning tree $T$ of $G$, with no cross-edges then the corresponding tree-augmentation LP, $LP(G, T)$ is integral.
\end{lemma}





